Magnetization reversal and anisotropies in buffered transition-metal alloys thin films

Interest in planar Hall effect (PHE) sensors has re-emerged in recent years due to their promising potential for a wide range of applications, particularly in biotechnology. Sensor sensitivity can be enhanced by lowering the effective anisotropy field; however, this favors magnetic domain formation during magnetization reversal, leading to hysteretic responses. Therefore, precise control of magnetic anisotropy and magnetization reversal is essential to balance sensitivity and stability in PHE sensors. In this work, we investigate the magnetic anisotropy and magnetization reversal mechanisms of Ni-Fe- and Co-Fe-based multilayers grown on various metallic buffer layers and deposited with and without an external magnetic field, in order to evaluate the effects of the buffer layers and field-assisted deposition on the resulting magnetic anisotropy. NiFe films exhibit a dominant uniaxial anisotropy mainly determined by the applied field during growth, with an anisotropy constant of approximately $3,\mathrm{kerg,cm^{-3}}$, largely independent of the buffer layer. In contrast, the magnetic anisotropy of CoFe films is dominated by the buffer layer, resulting in a biaxial magnetic response. In particular, Ag-buffered films deposited under an external magnetic field exhibit a biaxial anisotropy with values up to $14.88,\mathrm{kerg,cm^{-3}}$. The magnetization reversal mechanism of each system was deduced from the analysis of the angular dependence of the coercive field.

==> autores.tex <==
\author{A. Lo Giudice}
\affiliation{Instituto de Nanociencia y Nanotecnologia CNEA CONICET - Nodo Constituyentes, 1650 San Martin,  Buenos Aires, Argentina}

\author{A. Román}
\affiliation{Instituto de Nanociencia y Nanotecnologia CNEA CONICET - Nodo Constituyentes, 1650 San Martin,  Buenos Aires, Argentina}
\affiliation{Dpto. Micro y Nanotecnologia, Centro Atomico Constituyentes CNEA, 1650 San Martin, Buenos Aires, Argentina}

\author{L.B. Steren}
\affiliation{Instituto de Nanociencia y Nanotecnologia CNEA CONICET - Nodo Constituyentes, 1650 San Martin,  Buenos Aires, Argentina}

